Analysis and Synthesis of Low-Gain Integral Controllers for Nonlinear Systems

Relaxed conditions are given for stability of a feedback system consisting of an exponentially stable multi-input multi-output nonlinear plant and an integral controller. Roughly speaking, it is shown that if the composition of the plant equilibrium input-output map and the integral feedback gain is infinitesimally contracting, then the closed-loop system is exponentially stable if the integral gain is sufficiently low. The main result is illustrated with an application arising in frequency control of AC power systems. We demonstrate how the contraction condition can be checked computationally via semidefinite programming, and how integral gain matrices can be synthesized via convex optimization to achieve robust L2 performance in the presence of nonlinearity and uncertainty.

==> macros-commands.tex <==

%-----------------------------------------
%-------- Francesco's Commands -----------
%-----------------------------------------

\newcounter{myboard}
\setcounter{myboard}{1}

\newcommand{\board}[1]{\clearpage\begin{center}{%
%% \footnoterule\vspace{.5em}
\begin{minipage}[t]{0.9\linewidth}
  \Large Section \arabic{myboard}: #1 \end{minipage}\vspace{.5em}
\footnoterule}\end{center}\addtocounter{myboard}{1}\par}

\newcommand{\boardsubsec}[1]{\clearpage\begin{center}{%
%%\footnoterule\vspace{.5em}
\begin{minipage}[t]{0.9\linewidth}
  \Large Subsection \arabic{myboard}: #1 \end{minipage}\vspace{.5em}
\footnoterule}\end{center}\addtocounter{myboard}{1}\par}

\newcommand{\booktitle}{Robust Feedback Systems and Integral Quadratic Constraints}
\newcommand{\booktitlemain}{Robust Feedback Systems and Integral Quadratic Constraints}


%--------------------------------------------
%-------Color and Commenting Commands--------
%--------------------------------------------

\newcommand{\tr}{\color{red}}
\newcommand{\tv}{\color{violet}}
\newcommand{\tb}{\color{blue}}
\newcommand{\tg}[0]{\color{ForestGreen}}
\definecolor{myvar}{rgb}{0, 0.5, 0}
\newcommand{\var}[1]{\textcolor{myvar}{#1}}
\newcommand{\john}[1]{{\leavevmode\color{blue}\textbf{From John:\;}#1}}
\newcommand{\jstodo}[1]{\par\noindent{\color{blue} \centering From JWSP: $<<<$\textsf{#1}$>>>$  \par}}

\usepackage{marginnote}
\newcommand{\johnref}{\textbf{\textcolor{red}{[ref] }}}
\newcommand\fyimargin[1]{\marginpar{\color{violet} \small\ttfamily FYI (read and erase): #1}}
\newcommand{\todo}[1]{\par\noindent{\color{blue}\raggedright\textsc{#1}\par\marginpar{\large$\star$}}}
\newcommand{\fdmargin}[1]{\marginpar{\color{blue}\tiny\ttfamily{FD:} #1}}
\newcommand{\jsmargin}[1]{\marginpar{\color{red}\tiny\ttfamily{JS:} #1}}
\newcommand{\fbmargin}[1]{\marginpar{\color{red}\small\ttfamily{FB:} #1}}


%--------------------------------------------
%-------Mathematical Style commands--------
%--------------------------------------------

\newcommand{\myemph}[1]{\ensuremath{\textbf{\emph{#1}}}}
\renewcommand{\myemph}[1]{\textbf{\emph{#1}}}
\newcommand{\itememph}[1]{\ensuremath{\textbf{\emph{#1}}}}

\newcommand{\define}{\ensuremath{\triangleq}}
\newcommand{\oprocendsymbol}{\hbox{$\bullet$}}
\newcommand{\oprocend}{\relax\ifmmode\else\unskip\hfill\fi\oprocendsymbol}

\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}


%--------------------------------------------
%-------Sets and Vector Notation-------------
%--------------------------------------------

\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
\newcommand{\real}{\mathbb{R}}
\newcommand{\mycircle}{\ensuremath{\mathbb S^{1}}}
\newcommand{\sphere}{\ensuremath{\mathbb S}}
\newcommand{\torus}{\ensuremath{\mathbb T}}
\newcommand{\F}{\ensuremath{\mathbb{F}}}
\newcommand{\poly}{\mathbb{P}}
\newcommand{\ereal}{\real \union \{\infty\}}
\newcommand{\complex}{\mathbb{C}}
\newcommand{\integer}{\mathbb{Z}}
\newcommand{\disk}{\mathbb{D}}
\newcommand{\realpositive}{{\mathbb{R}}_{>0}}
\newcommand{\realnonnegative}{{\mathbb{R}}_{\geq 0}}
\newcommand{\integerspositive}{\mathbb{Z}_{\geq 1}}

\newcommand{\vect}[1]{\mathbbold{#1}}
\newcommand{\vones}[1][]{\vect{1}_{#1}}
\newcommand{\vzeros}[1][]{\vect{0}_{#1}}

\renewcommand{\Re}{\mathrm{Re}}
\renewcommand{\Im}{\mathrm{Im}}
\renewcommand{\deg}{\mathrm{deg}}
\DeclareMathOperator*{\Res}{\mathrm{Res}}

\newcommand{\diag}{\mathrm{diag}}
\newcommand{\daug}{\mathrm{daug}}

\newcommand{\ball}[2]{\mathscr{B}_{#1}(#2)}


%--------------------------------------------
%-------General Mathematics Functions--------
%--------------------------------------------

\renewcommand{\d}{\ensuremath{\mathrm{d}}}
\newcommand{\map}[3]{#1: #2 \rightarrow #3}
\DeclareMathOperator*{\esssup}{ess\,sup}
\newcommand{\dom}{\mathrm{dom}}
\newcommand{\T}{\mathsf{T}}
\renewcommand{\j}{\ensuremath{\mathbf{j}}}
\newcommand{\supscr}[2]{#1^{\textup{#2}}}				
\newcommand{\subscr}[2]{#1_{\textup{#2}}} % abbreviation for
\newcommand{\e}[1][]{\vect{e}_{#1}}

\newcommand{\nodes}{\mathcal{N}}
\newcommand{\edges}{\mathcal{E}}

\newcommand{\col}{\ensuremath{\mathrm{col}}}
\newcommand{\spec}{\ensuremath{\mathrm{spec}}}
\newcommand{\eig}{\ensuremath{\mathrm{eig}}}
\newcommand{\vspan}{\mathrm{span}}
\newcommand{\codim}{\mathrm{codim}}
\newcommand{\trace}{\mathrm{trace}}
\newcommand{\image}{\mathrm{image}}
\newcommand{\coker}{\mathrm{coker}}
\newcommand{\ind}{\mathrm{ind}}
\newcommand{\corank}{\mathrm{corank}}
\newcommand{\coimage}{\mathrm{coimage}}
\newcommand{\nullity}{\mathrm{nullity}}
\newcommand{\rank}{\mathrm{rank}}
\renewcommand{\char}{\ensuremath{\mathrm{char}}}

\DeclareMathOperator*{\intersection}{\cap}
\DeclareMathOperator*{\union}{\cup}
\DeclareMathOperator*{\bigintersection}{\ensuremath{\bigcap}}
\DeclareMathOperator*{\bigunion}{\ensuremath{\bigcup}} 

\newcommand{\id}{\ensuremath{\mathrm{id}}}
\newcommand{\graph}{\ensuremath{\mathrm{graph}}}
\newcommand{\supp}{\ensuremath{\mathrm{supp}}}

\newcommand{\conv}{\mathrm{conv}}
\newcommand{\affine}{\mathrm{affine}}
\newcommand{\relint}{\ensuremath{\mathrm{relint}}}
\newcommand{\interior}{\ensuremath{\mathrm{interior}}}
\newcommand{\closure}{\ensuremath{\mathrm{closure}}}
\newcommand{\boundary}{\ensuremath{\mathrm{bd}}}

\newcommand{\sym}[1]{\ensuremath{\mathbb{S}^{#1}}}
\newcommand{\her}[1]{\ensuremath{\mathbb{H}^{#1}}}
\newcommand{\pd}[1]{\ensuremath{\mathbb{S}_{>0}^{#1}}}
\newcommand{\psd}[1]{\ensuremath{\mathbb{S}_{\geq 0}^{#1}}}
\newcommand{\nd}[1]{\ensuremath{\mathbb{S}_{<0}^{#1}}}
\newcommand{\nsd}[1]{\ensuremath{\mathbb{S}_{\leq 0}^{#1}}}



\newcommand{\E}{\mathbb{E}}
\newcommand{\rms}{\ensuremath{\mathrm{rms}}}
\newcommand{\pow}{\ensuremath{\mathrm{pow}}}
\newcommand{\mean}{\ensuremath{\mathrm{mean}}}


%--------------------------------------------
%-------Norms and Inner Products-------------
%--------------------------------------------

\newcommand{\norm}[2]{\ensuremath{\|#1\|_{#2}}}
\newcommand{\bignorm}[1]{\ensuremath{\big \| #1 \big \|}}
\newcommand{\Bignorm}[1]{\ensuremath{\Big \| #1 \Big \|}}
\newcommand{\Biggnorm}[1]{\ensuremath{\Bigg \| #1 \Bigg \|}}

\newcommand{\setdef}[2]{\{#1 \;|\; #2\}}
\newcommand{\bigsetdef}[2]{\big\{#1 \;|\; #2\big\}}
\newcommand{\Bigsetdef}[2]{\Big\{#1 \;|\; #2\Big\}}
\newcommand{\Biggsetdef}[2]{\Bigg\{#1 \;|\; #2\Bigg\}}

\newcommand{\inner}[3]{\ensuremath{\langle #1,#2\rangle}_{#3}}
\newcommand{\Biginner}[3]{\ensuremath{\Big\langle #1,#2\Big\rangle}_{#3}}
\newcommand{\Bigginner}[3]{\ensuremath{\Bigg\langle #1,#2\Bigg\rangle}_{#3}}

\makeatletter
\newcommand{\vast}{\bBigg@{4}}
\newcommand{\Vast}{\bBigg@{5}}
\newcommand{\vastinner}[3]{\ensuremath{\vast\langle #1,#2\vast\rangle}_{#3}}
\newcommand{\Vastinner}[3]{\ensuremath{\Vast\langle #1,#2\Vast\rangle}_{#3}}


%--------------------------------------------
%-------Signal Spaces------------------------
%--------------------------------------------

\newcommand{\Fourier}{\ensuremath{\mathscr{F}}}
\newcommand{\InvFourier}{\ensuremath{\mathscr{F}^{-1}}}
\newcommand{\Laplace}{\ensuremath{\Lambda}}
\newcommand{\Laplacecausal}{\ensuremath{\Lambda^+}}
\newcommand{\Laplaceacausal}{\ensuremath{\Lambda^-}}

\newcommand{\Mult}[1]{\ensuremath{\mathsf{M}_{#1}}}
\newcommand{\Conv}[1]{\ensuremath{\mathsf{Conv}_{#1}}}

\newcommand{\ContrX}[1]{\ensuremath{\mathscr{C}_{r}({\real};#1)}}
\newcommand{\Contr}[1]{\ensuremath{\mathscr{C}_{r}^{#1}({\real})}}
\newcommand{\ContR}[2]{\ensuremath{\mathscr{C}_{#1}^{#2}({\real})}}
\newcommand{\ContC}[2]{\ensuremath{\mathscr{C}_{#1}^{#2}({\j\real})}}

\newcommand{\Tdist}{\ensuremath{\mathsf{T}}}
\newcommand{\Sch}{\ensuremath{\mathscr{S}(\real)}}
\newcommand{\Schcausal}{\ensuremath{\mathscr{S}[0,\infty)}}
\newcommand{\Schacausal}{\ensuremath{\mathscr{S}(-\infty,0]}}
\newcommand{\Schprime}{\ensuremath{\mathscr{S}^{\prime}(\real)}}
\newcommand{\Schprimecausal}{\ensuremath{\mathscr{S}^{\prime}[0,\infty)}}
\newcommand{\Schprimeacausal}{\ensuremath{\mathscr{S}^{\prime}(-\infty,0]}}

\newcommand{\SchprimeC}{\ensuremath{\mathscr{S}^{\prime}(\j\real)}}
\newcommand{\SchC}{\ensuremath{\mathscr{S}(\j\real)}}

\newcommand{\Contrcausal}[1]{\ensuremath{\mathscr{C}_{r}^{#1}[0,\infty)}}
\newcommand{\Contcausal}[2]{\ensuremath{\mathscr{C}_{#1}^{#2}[0,\infty)}}


\newcommand{\myL}{\mathcal{L}}

\newcommand{\Lone}{\ensuremath{\myL_{1}}}
\newcommand{\LoneR}[1]{\ensuremath{\myL_{1}^{#1}(\real)}}
\newcommand{\Lonecausal}[1]{\ensuremath{\myL_{1}^{#1}[0,\infty)}}
\newcommand{\Loneacausal}[1]{\ensuremath{\myL_{1}^{#1}(-\infty,0]}}

\newcommand{\Lonee}{\ensuremath{\myL_{1\mathrm{e}}}}
\newcommand{\LoneeR}[1]{\ensuremath{\myL_{1\mathrm{e}}^{#1}(\real)}}
\newcommand{\Loneecausal}[1]{\ensuremath{\myL_{1\mathrm{e}}^{#1}[0,\infty)}}
\newcommand{\Loneeacausal}[1]{\ensuremath{\myL_{1\mathrm{e}}^{#1}(-\infty,0]}}

\newcommand{\ellone}{\ensuremath{\ell_{1}}}
\newcommand{\elltwo}{\ensuremath{\ell_{2}}}
\newcommand{\ellinf}{\ensuremath{\ell_{\infty}}}

\newcommand{\Sig}[1]{\ensuremath{\mathsf{Sig}^{#1}(\real)}}
\newcommand{\SigC}[1]{\ensuremath{\mathsf{Sig}^{#1}(\j\real)}}
\newcommand{\Sigcausal}[1]{\ensuremath{\mathsf{Sig}^{#1}[0,\infty)}}
\newcommand{\Sigacausal}[1]{\ensuremath{\mathsf{Sig}^{#1}(-\infty,0]}}

\newcommand{\Ltwo}{\ensuremath{\myL_{2}}}
\newcommand{\LtwoR}[1]{\ensuremath{\myL_{2}^{#1}(\real)}}
\newcommand{\Ltwocausal}[1]{\ensuremath{\myL_{2}^{#1}[0,\infty)}}
\newcommand{\Ltwoacausal}[1]{\ensuremath{\myL_{2}^{#1}(-\infty,0]}}
\newcommand{\Ltwotaucausal}[1]{\ensuremath{\myL_{2}^{#1}[\tau,\infty)}}
\newcommand{\Ltwotauacausal}[1]{\ensuremath{\myL_{2}^{#1}(-\infty,\tau]}}
\newcommand{\LtwoTcausal}[1]{\ensuremath{\myL_{2}^{#1}[T,\infty)}}
\newcommand{\LtwoTacausal}[1]{\ensuremath{\myL_{2}^{#1}(-\infty,T]}}


\newcommand{\Ltwoe}{\ensuremath{\myL_{2\mathrm{e}}}}
\newcommand{\LtwoeR}[1]{\ensuremath{\myL_{2\mathrm{e}}^{#1}(\real)}}
\newcommand{\Ltwoecausal}[1]{\ensuremath{\myL_{2\mathrm{e}}^{#1}[0,\infty)}}
\newcommand{\Ltwoeacausal}[1]{\ensuremath{\myL_{2\mathrm{e}}^{#1}(-\infty,0]}}
\newcommand{\Ltwoetaucausal}[1]{\ensuremath{\myL_{2\mathrm{e}}^{#1}[\tau,\infty)}}
\newcommand{\Ltwoetauacausal}[1]{\ensuremath{\myL_{2\mathrm{e}}^{#1}(-\infty,\tau]}}
\newcommand{\LtwoeTcausal}[1]{\ensuremath{\myL_{2\mathrm{e}}^{#1}[T,\infty)}}
\newcommand{\LtwoeTacausal}[1]{\ensuremath{\myL_{2\mathrm{e}}^{#1}(-\infty,T]}}

\newcommand{\Linf}{\ensuremath{\myL_{\infty}}}
\newcommand{\LinfR}[1]{\ensuremath{\myL_{\infty}^{#1}(\real)}}
\newcommand{\Linfcausal}[1]{\ensuremath{\myL_{\infty}^{#1}[0,\infty)}}
\newcommand{\Linfacausal}[1]{\ensuremath{\myL_{\infty}^{#1}(-\infty,0]}}

\newcommand{\Linfe}{\ensuremath{\myL_{\infty\mathrm{e}}}}
\newcommand{\LinfeR}[1]{\ensuremath{\myL_{\infty\mathrm{e}}^{#1}(\real)}}
\newcommand{\Linfecausal}[1]{\ensuremath{\myL_{\infty\mathrm{e}}^{#1}[0,\infty)}}
\newcommand{\Linfeacausal}[1]{\ensuremath{\myL_{\infty\mathrm{E}}^{#1}(-\infty,0]}}

\newcommand{\Lp}{\ensuremath{\myL_{\rm p}}}
\newcommand{\LpR}[1]{\ensuremath{\myL_{\rm p}^{#1}(\real)}}
\newcommand{\Lpcausal}[1]{\ensuremath{\myL_{\rm p}^{#1}[0,\infty)}}
\newcommand{\Lpacausal}[1]{\ensuremath{\myL_{\rm p}^{#1}(-\infty,0]}}
\newcommand{\Lptaucausal}[1]{\ensuremath{\myL_{\rm p}^{#1}[\tau,\infty)}}
\newcommand{\Lptauacausal}[1]{\ensuremath{\myL_{\rm p}^{#1}(-\infty,\tau]}}


\newcommand{\Lpe}{\ensuremath{\myL_{\mathrm{pe}}}}
\newcommand{\LpeR}[1]{\ensuremath{\myL_{\mathrm{pe}}^{#1}(\real)}}
\newcommand{\Lpecausal}[1]{\ensuremath{\myL_{\mathrm{pe}}^{#1}[0,\infty)}}
\newcommand{\Lpeacausal}[1]{\ensuremath{\myL_{\mathrm{pe}}^{#1}(-\infty,0]}}
\newcommand{\Lpetaucausal}[1]{\ensuremath{\myL_{\mathrm{pe}}^{#1}[\tau,\infty)}}
\newcommand{\Lpetauacausal}[1]{\ensuremath{\myL_{\mathrm{pe}}^{#1}(-\infty,\tau]}}

\newcommand{\Lq}{\ensuremath{\myL_{\rm q}}}
\newcommand{\LqR}[1]{\ensuremath{\myL_{\rm q}^{#1}(\real)}}
\newcommand{\Lqcausal}[1]{\ensuremath{\myL_{\rm q}^{#1}[0,\infty)}}
\newcommand{\Lqacausal}[1]{\ensuremath{\myL_{\rm q}^{#1}(-\infty,0]}}

\newcommand{\Lqe}{\ensuremath{\myL_{\rm qe}}}
\newcommand{\LqeR}[1]{\ensuremath{\myL_{\rm qe}^{#1}(\real)}}
\newcommand{\Lqecausal}[1]{\ensuremath{\myL_{\rm qe}^{#1}[0,\infty)}}
\newcommand{\Lqeacausal}[1]{\ensuremath{\myL_{\rm qe}^{#1}(-\infty,0]}}

\newcommand{\Lr}{\ensuremath{\myL_{\rm r}}}
\newcommand{\LrR}[1]{\ensuremath{\myL_{\rm r}^{#1}(\real)}}
\newcommand{\Lrcausal}[1]{\ensuremath{\myL_{\rm r}^{#1}[0,\infty)}}
\newcommand{\Lracausal}[1]{\ensuremath{\myL_{\rm r}^{#1}(-\infty,0]}}

\newcommand{\Lre}{\ensuremath{\myL_{\rm re}}}
\newcommand{\LreR}[1]{\ensuremath{\myL_{\rm re}^{#1}(\real)}}
\newcommand{\Lrecausal}[1]{\ensuremath{\myL_{\rm re}^{#1}[0,\infty)}}
\newcommand{\Lreacausal}[1]{\ensuremath{\myL_{\rm re}^{#1}(-\infty,0]}}

\newcommand{\hatLp}{\ensuremath{\hat{\myL}_{\rm p}}}
\newcommand{\hatLpC}[1]{\ensuremath{\hat{\myL}_{\rm p}^{#1}(\j\real)}}

\newcommand{\hatLq}{\ensuremath{\hat{\myL}_{\rm q}}}
\newcommand{\hatLqC}[1]{\ensuremath{\hat{\myL}_{\rm q}^{#1}(\j\real)}}

\newcommand{\hatLone}{\ensuremath{\hat{\myL}_{1}}}
\newcommand{\hatLoneC}[1]{\ensuremath{\hat{\myL}_{1}^{#1}(\j\real)}}

\newcommand{\hatLtwo}{\ensuremath{\hat{\myL}_{2}}}
\newcommand{\hatLtwoC}[1]{\ensuremath{\hat{\myL}_{2}^{#1}(\j\real)}}

\newcommand{\hatLinf}{\ensuremath{\hat{\myL}_{\infty}}}
\newcommand{\hatLinfC}[1]{\ensuremath{\hat{\myL}_{\infty}^{#1}(\j\real)}}

\newcommand{\trunc}[1]{\ensuremath{\mathcal{T}_{#1}}}
\newcommand{\projacausal}[1]{\ensuremath{\mathcal{P}_{(-\infty,#1]}}}
\newcommand{\projcausal}[1]{\ensuremath{\mathcal{P}_{[#1,\infty)}}}
\newcommand{\PT}{\ensuremath{\mathcal{P}_{T}}}
\renewcommand{\P}[1]{\ensuremath{\mathcal{P}_{#1}}}
\newcommand{\Ptau}{\ensuremath{\mathcal{P}_{\tau}}}
\newcommand{\shift}[1]{\ensuremath{\mathcal{S}_{#1}}}

\newcommand{\Hinf}{\ensuremath{\mathcal{H}_{\infty}}}
\newcommand{\HinfC}[1]{\ensuremath{\mathcal{H}_{\infty}^{#1}(\j\real)}}
\newcommand{\Htwo}{\ensuremath{\mathcal{H}_{2}}}
\newcommand{\HtwoC}[1]{\ensuremath{\mathcal{H}_{2}^{#1}(\j\real)}}

\newcommand{\Rat}{\ensuremath{\mathcal{R}}}
\newcommand{\RHinf}{\ensuremath{\mathcal{RH}_{\infty}}}
\newcommand{\RHinfC}[1]{\ensuremath{\mathcal{RH}_{\infty}^{#1}(\j\real)}}
\newcommand{\RHtwo}{\ensuremath{\mathcal{RH}_{2}}}
\newcommand{\RHtwoC}[1]{\ensuremath{\mathcal{RH}_{2}^{#1}(\j\real)}}
\newcommand{\RhatLtwoC}[1]{\ensuremath{\mathcal{R}\hat{\myL}_{2}^{#1}(\j\real)}}


\newcommand{\forallt}{\ensuremath{\text{for all}\,\,\,t \geq 0}}
\newcommand{\step}{\ensuremath{\mathsf{1}}}

\newcommand{\Test}{\ensuremath{\mathscr{D}}}
\newcommand{\pv}[1]{\ensuremath{\mathsf{pv}\left(\frac{1}{#1}\right)}}

%--------------------------------------------
%-------Robust Control Notation--------------
%--------------------------------------------

\newcommand{\rmodel}[4]{
            \left[
            \begin{array}{c|c}
                {#1} & {#2}\\
                \hline
                {#3} & {#4}
            \end{array}
            \right]
}

\newcommand{\IQC}{\mathsf{IQC}}
\newcommand{\SIQC}{\mathsf{SIQC}}
\newcommand{\HIQC}{\mathsf{HIQC}}

\newcommand{\hatPi}{\hat{\Pi}}
\newcommand{\hatPsi}{\hat{\Psi}}

\newcommand{\sector}{\mathtt{sector}}
\newcommand{\slope}{\mathtt{slope}}
\newcommand{\sat}{\mathsf{sat}}

\newcommand{\matlab}{\texttt{MATLAB}\,\,}

\newcommand{\CallierR}[1]{\mathscr{A}_{#1}(\real)}
\newcommand{\Calliercausal}[1]{\mathscr{A}_{#1}[0,\infty)}
\newcommand{\Callieracausal}[1]{\mathscr{A}_{#1}(-\infty,0]}
\newcommand{\hatCallier}[1]{\hat{\mathscr{A}}_{#1}}


%--------------------------------------------
%-------MathSF sets and subspaces------------
%--------------------------------------------

\newcommand{\V}{\ensuremath{\mathsf{V}}}
\newcommand{\Ps}{\ensuremath{\mathsf{P}}}
\newcommand{\Qs}{\ensuremath{\mathsf{Q}}}
\newcommand{\basis}[1]{\ensuremath{\mathscr{B}_{#1}}}
\renewcommand{\U}{\ensuremath{\mathsf{U}}}
\newcommand{\Y}{\ensuremath{\mathsf{Y}}}
\newcommand{\A}{\ensuremath{\mathsf{A}}}
\newcommand{\X}{\ensuremath{\mathsf{X}}}
\renewcommand{\C}{\ensuremath{\mathsf{C}}}
\newcommand{\K}{\ensuremath{\mathsf{K}}}
\newcommand{\D}{\ensuremath{\mathsf{D}}}
\newcommand{\W}{\ensuremath{\mathsf{W}}}
\newcommand{\Z}{\ensuremath{\mathsf{Z}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calU}{\ensuremath{\mathcal{V}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\I}{\ensuremath{I}}


% -------------------------------------
% ---------- Optimization Commands ----
% -------------------------------------

\newcommand{\card}{\mathop{\bf card}}
\newcommand{\prox}{\mathbf{prox}}

\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize} 	
\DeclareMathOperator*{\find}{find} 	
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\epi}{\mathop{\rm epi}}








